Boosting Object Detection with Zero-Shot Day-Night Domain Adaptation

Detecting objects in low-light scenarios presents a persistent challenge, as detectors trained on well-lit data exhibit significant performance degradation on low-light data due to low visibility. Previous methods mitigate this issue by exploring image enhancement or object detection techniques with real low-light image datasets. However, the progress is impeded by the inherent difficulties about collecting and annotating low-light images. To address this challenge, we propose to boost low-light object detection with zero-shot day-night domain adaptation, which aims to generalize a detector from well-lit scenarios to low-light ones without requiring real low-light data. Revisiting Retinex theory in the low-level vision, we first design a reflectance representation learning module to learn Retinex-based illumination invariance in images with a carefully designed illumination invariance reinforcement strategy. Next, an interchange-redecomposition-coherence procedure is introduced to improve over the vanilla Retinex image decomposition process by performing two sequential image decompositions and introducing a redecomposition cohering loss. Extensive experiments on ExDark, DARK FACE, and CODaN datasets show strong low-light generalizability of our method. Our code is available at https://github.com/ZPDu/DAI-Net.

==> Fig/enhance.tex <==
\begin{figure*}[!t]

% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=\textwidth]{Fig/enhance_.pdf}

\caption{ Left: Decomposition examples on DARK FACE.
}
\label{fig:enhance}

\end{figure*}

==> Tab/ablation.tex <==
\begin{wraptable}{R}{0.5\textwidth}
	\vspace{-0.2in}
	\scriptsize
 % \footnotesize	
  \centering
	\caption{Ablation Study of proposed components on DARK FACE.}
	% \vspace{0.05in}

	\label{table:ablation}
	{
		\begin{sc}
			\begin{tabular}{ccccc|c}
				\toprule
				\multicolumn{5}{c|}{Method} & \multirow{2}{*}{mAP(\%)}  \\\cmidrule{1-5}
                LLDP & RAL & $\mathcal{L}_{dec}$&$\mathcal{L}_{red}$ & $\mathcal{L}_{mc}$ & \\
				\midrule

                -- & --& --& -- & -- & 15.2 \\
                \checkmark & --& --& -- & --&11.6\\
                \checkmark & \checkmark & -- & -- & --& 20.5\\
                \checkmark & \checkmark & \checkmark & -- & -- & 21.8\\
                \checkmark & \checkmark & \checkmark & \checkmark & -- & 22.0\\
                \checkmark & \checkmark & -- & \checkmark & -- &  22.3\\
                \checkmark & \checkmark & --& \checkmark & \checkmark & \textbf{23.5}\\
                 \bottomrule
			\end{tabular}
		\end{sc}
	}
	% \vspace{-0.3in}
\end{wraptable}

==> Tab/abonrdlosses.tex <==
\begin{table}[h]

\centering
    % \scriptsize
    % \setlength{\tabcolsep}{2.5mm}
    % \vspace{-5px}
    % \resizebox{\linewidth}{!}{

	\begin{tabular}{c|c}
    
		\toprule
		Method & mAP(\%)\\
	\midrule
        Baseline & 15.2\\
        \midrule
        +$\mathcal{L}_{ref}$ & \\
        +$\mathcal{L}_{recon}$ & \\
        +$\mathcal{L}_{smooth}$ & \\
        +$\mathcal{L}_{ir}$ & 20.5\\
    \bottomrule
	\end{tabular}
    % }
    % \vspace{-10px}
	
    	\caption{Parameter variation ($M, N$) in reflectance decoder.}
\label{tab:ablationreflosses}

\end{table}


==> Tab/compface.tex <==
\begin{wraptable}{R}{0.5\textwidth}
	% \vspace{-0.3in}
	\scriptsize
 % \footnotesize	
  \centering
	\caption{Comparison with state-of-the-art methods on DARK FACE Test set.}
	% \vspace{0.05in}

	\label{table:darkface}
	{
		\begin{sc}
			\begin{tabular}{l|l|c}
				\toprule
				Category & {Method} & {mAP(\%)}  \\
				\midrule
                \multirow{7}{*}{Generalization} & Faster-RCNN~\cite{ren2015nips} & 1.7\\
                & SSH~\cite{najibi2017iccv} & 6.9\\
                & RetinaFace~\cite{deng2020cvpr}& 8.6\\
                & SRN~\cite{chi2019aaai} & 9.0\\
                & SFA~\cite{luo2019access} & 9.3\\
                & ParamidBox~\cite{tang2018eccv} & 12.5\\
                & SmallHardFace~\cite{zhang2020wacv} & 16.1\\
                & DSFD~\cite{li2019cvpr}& 16.1\\
                 & \textbf{Ours} & \textbf{28.0}\\
				\midrule
                \multirow{1}{*}{Enhancement} &DSFD+SCI~\cite{ma2022cvpr} & 34.8\\
                & \textbf{Ours+SCI}~\cite{ma2022cvpr}&\textbf{37.9}\\
                \midrule
                % \multirow{2}{*}{Unsuperwised DA} & HLA-Face~\cite{wang2021cvpr} & 44.4\\
                %  & \textbf{Adapted IIDet}&  \\
                % \midrule
                \multirow{2}{*}{Fully Supervised} & Fine-tuned DSFD~\cite{wang2021cvpr}& 46.0\\
                 & \textbf{Fine-tuned IIDet}& \textbf{52.9}\\
                 \bottomrule
			\end{tabular}
		\end{sc}
	}
	% \vspace{-0.4in}
\end{wraptable}

==> Tab/suppdecomnet.tex <==
\begin{table}[t]

\begin{minipage}{0.49\linewidth}
    
\centering
    % \scriptsize
    % \setlength{\tabcolsep}{2.5mm}
    % \vspace{-5px}
    % \resizebox{\linewidth}{!}{

	\begin{tabular}{c|c}
    
		\toprule
		Method & mAP(\%)\\
	\midrule
        Ours & 23.5\\
        w/ RF & 24.2\\
    \bottomrule
	\end{tabular}
    % }
    % \vspace{-10px}

    	\caption{Alternative of Retinex decomposition net.}

\label{tab:ablationdecomnet}

\end{minipage}
\hfill
\begin{minipage}{0.49\linewidth}
    
\centering
    % \scriptsize
    % \setlength{\tabcolsep}{2.5mm}
    % \vspace{-5px}
    % \resizebox{\linewidth}{!}{

	\begin{tabular}{c|c}
    
		\toprule
		Method & mAP(\%)\\
	\midrule
        HLA-Face & 44.4\\
        Ours & 44.8\\
    \bottomrule
	\end{tabular}
    % }
    % \vspace{-10px}

    	\caption{Comparison in unsupervised domain adaptation.}
  
\label{tab:compda}

\end{minipage}

\end{table}

